The Optimal Mechanism in Differential Privacy

We derive the optimal $\epsilon$-differentially private mechanism for single real-valued query function under a very general utility-maximization (or cost-minimization) framework. The class of noise probability distributions in the optimal mechanism has {\em staircase-shaped} probability density functions which are symmetric (around the origin), monotonically decreasing and geometrically decaying. The staircase mechanism can be viewed as a {\em geometric mixture of uniform probability distributions}, providing a simple algorithmic description for the mechanism. Furthermore, the staircase mechanism naturally generalizes to discrete query output settings as well as more abstract settings. We explicitly derive the optimal noise probability distributions with minimum expectation of noise amplitude and power. Comparing the optimal performances with those of the Laplacian mechanism, we show that in the high privacy regime ($\epsilon$ is small), Laplacian mechanism is asymptotically optimal as $\epsilon \to 0$; in the low privacy regime ($\epsilon$ is large), the minimum expectation of noise amplitude and minimum noise power are $\Theta(\Delta e^{-\frac{\epsilon}{2}})$ and $\Theta(\Delta^2 e^{-\frac{2\epsilon}{3}})$ as $\epsilon \to +\infty$, while the expectation of noise amplitude and power using the Laplacian mechanism are $\frac{\Delta}{\epsilon}$ and $\frac{2\Delta^2}{\epsilon^2}$, where $\Delta$ is the sensitivity of the query function. We conclude that the gains are more pronounced in the low privacy regime.

==> discussion.tex <==
In this section, we discuss our results and compare them with other related works.

\subsection{Laplacian Mechanism vs Staircase Mechanism}

The Laplacian mechanism is specified by two parameters, $\e$ and the query function sensitivity $\D$. $\e$ and $\D$ completely characterize the  differential privacy constraint \eqref{eqn:dpconstraintfinal}. On the other hand, our staircase mechanism is specified by three parameters, $\e$, $\D$, and $\gamma^*$ which is determined by $\e$ and the cost function $\loss(\cdot)$. For certain classes of cost functions $\loss(\cdot)$, there are closed-form expressions for the optimal $\gamma^*$.

From the two examples given in Section \ref{sec:application}, we can see that although Laplacian mechanism is not strictly optimal, in the high privacy regime ($\e \to 0$), Laplacian mechanism is asymtotically optimal: \begin{itemize}
	\item for $L(x) = |x|$, the additive gap from the optimal values goes to 0 as $\e \to 0$,
	\item for $L(x) = x^2$, the additive gap from the optimal values is upper bounded by a constant  as $\e \to 0$.
\end{itemize}
 However, in the low privacy regime ($\e \to +\infty$), the multiplicative gap from the optimal values can be arbitrarily large. We conclude that in high privacy regime Laplacian mechanism is nearly optimal, while in low privacy regime significant improvement can be achieved by using staircase mechanism. We plot the multiplicative gain of Staircase mechanism over Laplacian mechanism for cost functions $\loss(x) = |x|$ and $\loss(x) = x^2$ in Figure  \ref{fig:comparison}. We can see that even for modest $\e \approx 10$, staircase mechanism has about 15-fold and 23-fold improvement.
 
Since our staircase mechanism is derived under the same problem setting with Laplacian mechanism, staircase mechanism can be applied wherever Laplacian mechanism is used, and it performs strictly better than Laplacian mechanism.



\begin{figure}[h]
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.1\textwidth]{fig1.pdf}
\caption{ $0 < \e \le 10 $}
\label{fig:compare1}
\end{subfigure}
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.1\textwidth]{fig2.pdf}
\caption{ $10 \le \e \le 20$}
\label{fig:compare2}
\end{subfigure}
\caption{Multiplicative Gain of Staircase Mechanism over Laplacian Mechanism}
\label{fig:comparison}
\end{figure}




% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.2]{comparison.pdf}
% \caption{Multiplicative Gain of Staircase Mechanism over Laplacian Mechanism}
% \label{fig:comparison}
% \end{figure}


\subsection{Worst-case Result}

We emphasize that our staircase mechanism is a worst-case optimal result. We impose no further assumptions on the properties of query function $q$ beyond its sensitivity. If we know more properties  $q$ satisfies, it is entirely possible that  staircase mechanism is not the best. For example, if we know the range of $q$ is $\Z$, then we even do not need to add noise which are not integers, in which case discrete probability distributions are the best.

\subsection{Relation to Ghosh et. al. \cite{Ghosh09}}

There are some excellent works on studying noise distributions in differential privacy, e.g., \cite{geometry} and \cite{Ghosh09}. One of the most well-know result is \cite{Ghosh09}, which shows geometric mechanism, a discrete variant of Laplacian mechanism, is optimal for single count query function.

The difference between our work and \cite{Ghosh09} is
\begin{itemize}
	\item \cite{Ghosh09} studies count query function, which is integer-valued, while we study general real-valued query function. Therefore, the geometric mechanism in \cite{Ghosh09} add integer-valued noise, while our staircase mechanism add real-valued noise and has continuous probability distribution.

	\item In \cite{Ghosh09}  the sensitivity of count query function is one, i.e, $\D = 1$, while in our work there is no constraint on $\D$. From the proof of Theorem \ref{thm:main}, it is easy to see for integer-valued query function with  $\D \ge 2$, the optimal noise probability mass function  is also staircase-shaped, which can be viewed as a discrete variant of staircase mechanism.  In the case $\D =1$, the staircase-shaped probability mass function is reduced to corresponding to a strictly decreasing geometric series.
\end{itemize} 


	% \subsection{Remove Property \ref{property2}}

	% Our optimality result holds for a general class of cost functions which satisfies Property \ref{propert1} and Property \ref{propert2}. We believe we can remove constraint property2.

==> formulation.tex <==

Consider a real-valued query function
\begin{align}
	q: \database \rightarrow \R,
\end{align}
where $\database$ is the domain of the databases.

The sensitivity of the query function $q$ is defined as
\begin{align}
	\D \triangleq \max_{ D_1,D_2 \subseteq \database: |D_1 - D_2| \le 1} | q(D_1) - q(D_2)|, \label{def:sensitivity}
\end{align}
where the maximum is taken over all possible pairs of neighboring database entries $D_1$ and $D_2$ which differ in at most one element, i.e., one is a proper subset of the other and the larger database contains just one additional element \cite{DPsurvey}.

\begin{definition}[$\e$-differential privacy \cite{DPsurvey}]
	A randomized mechanism $\KM$ gives $\e$-differential privacy if for all data sets $D_1$ and $D_2$ differing on at most one element, and all $S \subset \text{Range}(\KM)$,
	\begin{align}
	 	\text{Pr}[\KM(D_1) \in S] \le \exp(\e) \;  \text{Pr}[\KM(D_2) \in S]. \label{eqn:dpgeneral}
	 \end{align}
\end{definition}


The standard approach to preserving the differential privacy is to add noise to the output of query function. Let $q(D)$ be the value of the query function evaluated at $D \subseteq \database$, the noise-adding  mechanism $\KM$ will output
\begin{align}
 	\KM(D) = q(D) + \noise,
 \end{align}
where $\noise$ is the noise added by the mechanism to the output of query function.

In the following we derive the differential privacy constraint on the probability distribution of $\noise$ from \eqref{eqn:dpgeneral}.
\begin{alignat}{2}
	 & \; \text{Pr}[\KM(D_1) \in S] & &\le  \exp(\e)\; \text{Pr}[\KM(D_2) \in S] \\
	 \Leftrightarrow & \; \text{Pr}[ q(D_1) + \noise \in S]  & &\le \exp(\e) \; \text{Pr}[q(D_2) + \noise \in S] \\
	 \Leftrightarrow & \; \text{Pr}[  \noise \in S - q(D_1) ]  & &\le \exp(\e) \; \text{Pr}[  \noise \in S - q(D_2) ] \\
	 \Leftrightarrow & \; \text{Pr}[  \noise \in S' ] & &\le \exp(\e) \; \text{Pr}[  \noise \in S' + q(D_1)- q(D_2) ],  \label{eqn:dpconstraint2}
\end{alignat}
where $S' \triangleq S - q(D_1) = \{ s-q(D_1) | s \in S \}$.

%%%%%%%%%%%%%%%%%%%%% define S + d %%%%%%%%%%%%%%%%%%%%%


Since \eqref{eqn:dpgeneral} holds for all measurable sets $S \subseteq \R$, and $|q(D_1)- q(D_2)| \le \D$, from \eqref{eqn:dpconstraint2} we have
\begin{align}
	\text{Pr}[  \noise \in S' ] \le \exp(\e) \; \text{Pr}[  \noise \in S' + d], \label{eqn:dpconstraint3}
\end{align}
for all measurable sets $S' \subseteq \R$ and for all $|d| \le \D$.

Consider a cost function $\loss(\cdot)$ which is a function of the added noise $\noise$. Our goal is to minimize the expectation of the cost subject to the $\e$-differential privacy constraint \eqref{eqn:dpconstraint3}.

More precisely, let $\p$ denote the probability distribution of $\noise$ and use $\p(S)$ denote the probability $\text{Pr}[\noise \in S]$. The optimization problem we study in this paper is

\begin{align}
	\mathop{\text{minimize}}\limits_{ \p} & \ \int_{x \in \R} \loss(x) \p (dx) \\
	\text{subject to} & \ \p(S) \le e^{\e} \p(S + d), \forall \ \text{measurable set} \ S\subseteq \R, \ \forall |d| \le \D.  \label{eqn:dpconstraintfinal}
\end{align}

Our main contribution is to solve the above functional optimization problem and derive the optimal noise probability distribution for a general class of cost functions $\loss(\cdot)$.




==> introduction_backup_quan_20131030.tex <==

% Due to the advances of information technology and the prevalence of social networks, vast amounts of personal information can be efficiently collected and processed.  The availability of such \emph{big data} enables us produce a number of useful applications by analyzing the collected information. To make full use of the collected information, the data collector will release the information to other third-parties(analysts) to do data analysis and produce useful applications.

% While releasing the collected data has great potential use for analysis, without proper statistical disclosure mechanisms, the privacy of individuals in the dataset can be jeopardized. In 2006, Netflix hosted the Netflix prize contest, an open competition in which contestants design algorithms to make predictions on user ratings for movies from the released dataset by Netflix. The training dataset provided by Netflix consisted of 100,480,507   ratings that 480,189 users gave to  17,770 movies \cite{wikiNetflix}. To protect the privacy of customers in the released training dataset, Netflix anonymized the dataset by removing users' personal information, e.g., name, from the dataset, and only used integer IDs. However, these anonymization approaches were not sufficient to preserve customers' privacy. By connecting the released anonymized dataset by Netflix and the Internet Movie Database as background knowledge, Narayanan and Shmatikov \cite{netflix} successfully de-anonymize and identify some  Netflix records of known users.


% As can be seen from the Netflix Prize example, one difficulty to define a notion of \emph{privacy} which is resilient to attacks is to model the side information of adversaries. To preserve the privacy resilient to attacks with arbitrary side information, the only way is to use randomized data releasing mechanisms.

Differential privacy is a  formal framework to quantify to what extent individual privacy in a statistical database is preserved while releasing useful aggregate information about the database.
It provides strong privacy guarantees by requiring the indistinguishability of whether an individual is in the dataset or not based on the released information. The key idea of differential privacy is that the presence or absence
of any individual data in the database should not affect the final released statistical information significantly, and thus it can give strong privacy guarantees against an adversary with arbitrary auxiliary information. For motivation and background of differential privacy, we refer the readers to the  survey \cite{DPsurvey} by Dwork.

Since its introduction in \cite{DMNS06} by Dwork et.\ al., differential privacy has become the standard notion of privacy in releasing query output information for statistical databases and spawned  a large body of research in  differentially private data-releasing mechanism design and performance analysis in various settings. Differential privacy is a privacy-preserving constraint imposed on the query output releasing mechanisms, and to make use of the released information, it is important to understand the fundamental tradeoff between utility(accuracy) and privacy.



In many existing works on studying the tradeoff between accuracy and privacy in differential privacy, the usual metric of accuracy is in terms of the variance, or magnitude expectation of the noise added to the query output.  For example, Hardt and Talwar \cite{geometry} study the tradeoff between privacy and error for answering a set of linear queries over a histogram in a differentially private way, where the error is defined as the worst  expectation of the $\ell^2$-norm of the noise among all possible query output.  \cite{geometry} derives lower and upper bounds on the error given the differential privacy constraint. Nikolov, Talwar and Zhang \cite{NTZ12} extend the result on the tradeoff between privacy and error to the case of  $(\e,\delta)$-differential privacy. Li et. al. \cite{Li10} study how to optimize linear counting queries under differential privacy, where the error is measured by the mean squared error of query output estimates, which corresponds to the variance of the noise added to the query output to preserve differential privacy.

More generally, the error can be a general function depending on the additive noise (distortion) to the query output.  Ghosh, Roughgarden,  and Sundararajan \cite{Ghosh09}  study a very general utility-maximization framework for a single count query with sensitivity one under differential privacy, where the utility (cost) function can be a general function depending on the noise added to the query output. \cite{Ghosh09} shows that there exists a universally optimal mechanism (adding geometric noise) to preserve differential privacy for a general class of utility functions under a Bayesian framework.  Brenner and Nissim \cite{Nissim10} show that for general query functions, no universally optimal differential privacy mechanisms exist. Gupte and Sundararajan  \cite{minimax10} generalize the result of \cite{Ghosh09}  to a minimax setting.


In this work, we study the fundamental tradeoff between utility and privacy under differential privacy, and derive the optimal differentially private mechanism for  general single real-valued query function, where the utility model is the same as the one adopted in \cite{Ghosh09} and \cite{minimax10}, and the real-valued query function can have arbitrary sensitivity.  Our results can be viewed as a generalization of  \cite{Ghosh09} and \cite{minimax10} to general real-valued query functions with arbitrary sensitivity. We discuss the relations of our work and the existing works in detail in Section \ref{subsec:connection}.



\subsection{Background on Differential Privacy}

The basic problem setting in differential privacy for statistical database is as follows: suppose a dataset curator is in charge of a statistical database which consists of records of many individuals, and an analyst sends a query request to the curator to get some aggregate information about the whole database. Without any privacy concerns, the database curator can simply apply the query function to the dataset, compute the query output, and send the result to the analyst. However, to protect the privacy of individual data in the dataset, the dataset curator should use a randomized query-answering mechanism such that the probability distribution of the query output does not differ too much whether any individual record is in the database or not.

Formally, consider a real-valued query function
\begin{align}
	q: \database \rightarrow \R,
\end{align}
where $\database$ is the set of all possible datasets. The real-valued query function $q$ will be applied to a dataset, and query output is a real number. Two datasets $D_1, D_2 \in \database$ are called neighboring datasets if they differ in at most one element, i.e.,  one is a proper subset of the other and the larger dataset contains just one additional element \cite{DPsurvey}. A randomized query-answering mechanism $\KM$ for the query function $q$ will randomly output a number with probability distribution depends on query output $q(D)$, where $D$ is the dataset.

\begin{definition}[$\e$-differential privacy \cite{DPsurvey}]
	A randomized mechanism $\KM$ gives $\e$-differential privacy if for all data sets $D_1$ and $D_2$ differing on at most one element, and all $S \subset \text{Range}(\KM)$,
	\begin{align}
	 	\text{Pr}[\KM(D_1) \in S] \le \exp(\e) \;  \text{Pr}[\KM(D_2) \in S], \label{eqn:dpgeneral}
	 \end{align}
	 where $\KM(D)$ is the random output of the  mechanism $\KM$ when the query function $q$ is applied to the dataset $D$.
\end{definition}


The differential privacy constraint \eqref{eqn:dpgeneral} essentially requires that for all neighboring datasets, the probability distributions of the output of the randomized mechanism should be approximately the same. Therefore, for any individual record, its presence or absence in the dataset will not significantly affect the output of the mechanism, which makes it hard for adversaries with arbitrary background knowledge to make inference on any individual from the released query output information. The parameter $\e \in (0, +\infty)$ quantifies how private the mechanism is: the smaller $\e$ is , the more private the randomized mechanism is.



%%%%%%%%%  hypothesis testing context %%%%%%%%%


\subsubsection{Operational Meaning of $\e$-Differential Privacy in the Context of Hypothesis Testing}


As shown by \cite{Zhou08}, one can interpret the   differential privacy constraint  \eqref{eqn:dpgeneral} in the context of hypothesis testing in terms of false alarm probability and missing detection probability. Indeed, consider a binary hypothesis testing problem over two neighboring datasets, $H_0: D_1 $ versus $H_1: D_2$, where an individual's record is in $D_2$ only. Given a decision rule, let $S$ be the decision region such that when the released output lies in $S$, $H_1$ will be rejected, and when the released output lies in $S^C$ (the complement of $S$), $H_0$ will be rejected. The false alarm probability $P_{FA}$ and the missing detection probability $P_{MD}$ can be written as
\begin{align}
	P_{FA} &= P(K(D_1) \in S^C), \\
	P_{MD} &= P(K(D_2) \in S).
\end{align}

Therefore, from \eqref{eqn:dpgeneral} we get
\begin{align}
	1 - P_{FA} \le e^{\e} P_{MD} .
\end{align}
Thus
\begin{align}
	 e^{\e} P_{MD} + P_{FA} \ge 1 .
\end{align}

Switch $D_1$ and $D_2$ in \eqref{eqn:dpgeneral}, and we get
	\begin{align}
	 	\text{Pr}[\KM(D_2) \in S] \le \exp(\e) \;  \text{Pr}[\KM(D_1) \in S] .
	 \end{align}

Therefore,
\begin{align}
	1 - P_{MD} \le e^{\e} P_{FA} ,
\end{align}
and thus
\begin{align}
	 P_{MD} + e^{\e} P_{FA} \ge 1 .
\end{align}

In conclusion,  we have
\begin{align}
  e^{\e} P_{MD} + P_{FA} &\ge 1 , \\
	P_{MD} + e^{\e} P_{FA} &\ge 1 .
\end{align}

The $\e$-differential privacy constraint implies that in the context of hypothesis testing,  $P_{FA}$ and $P_{MD}$ can not be both too small. We plot the regions of $P_{FA}$ and $P_{MD}$ under $\e$-differential privacy in Figure \ref{fig:famd}.

\begin{figure}[t]
\centering
\includegraphics[scale=0.6]{fig_codes/epsilon_figure.pdf}
\caption{The Region of $P_{FA}$ and $P_{MD}$ under $\e$-Differential Privacy}
\label{fig:famd}
\end{figure}



%%%%%%%%%%%%%%%%%%%


\subsubsection{Laplacian Mechanism}



The standard approach to preserving $\e$-differential privacy is to perturb the query output by adding random noise with Laplacian distribution proportional to the sensitivity $\Delta$ of the query function $q$, where the  sensitivity of a real-valued query function is defined as

\begin{definition}[Query Sensitivity \cite{DPsurvey}]
	For a real-valued query function $q: \database \rightarrow \R$, the sensitivity of $q$ is defined as
	\begin{align}
	\D := \max_{D_1,D_2 \in \database} | q(D_1) - q(D_2)|, \label{def:sensitivity}
\end{align}
for all $D_1,D_2$ differing in at most one element.
\end{definition}


Formally, the  Laplacian mechanism is:
\begin{definition}[Laplacian Mechanism \cite{DMNS06}]
	For a real-valued query function $q: \database \rightarrow \R$ with sensitivity $\Delta$, Laplacian mechanism will output
	\begin{align}
		K(D) := q(D) + \text{Lap}(\frac{\D}{\e}),
	\end{align}
 	where $\text{Lap}(\lambda)$ is a random variable with probability density function
 	\begin{align}
 		f(x) = \frac{1}{2\lambda} e^{-\frac{|x|}{\lambda}}, \quad \forall x \in \R.
 	\end{align}
\end{definition}



%%%%%%%%%%%%%%%%%% add miss detection false alarm region for Laplacian mechanism  %%%%%%%%

Consider two neighboring datasets $D_1$ and $D_2$ where $|q(D_1) - q(D_2)| = \D$. It is easy to compute the tradeoff between the false alarm probability $P_{FA}$ and the missing detection probability $P_{MD}$  under  Laplacian mechanism, which is 
\begin{align}
P_{MD}  =
\begin{cases}
1 - e^{\e}P_{FA} & P_{FA} \in [0,   \frac{1}{2} e^{-\e}) \\
\frac{e^{-\e}}{4P_{FA}}  & P_{FA} \in [ \frac{1}{2} e^{-\e}, \frac{1}{2} ) \\
e^{-\e}(1 - P_{FA} ) & P_{FA} \in [\frac{1}{2}, 1] 
\end{cases}\label{eqn:regionLap}
\end{align}

The region of $P_{FA}$ and $F_{MD}$ under Laplacian mechanism for two neighboring datasets $D_1$ and $D_2$ such that $|q(D_1) - q(D_2)| = \D$ is ploted in Figure \ref{fig:regionLap}.


\begin{figure}[t]
\centering
\includegraphics[scale=0.6]{fig_codes/Laplace_figure.pdf}
\caption{The Region of $P_{FA}$ and $P_{MD}$ under Laplacian Mechanism}
\label{fig:regionLap}
\end{figure}

%%%%%%%%%%%%%%%%%% end %%%%%%%%%%%%%%%



Since its introduction in \cite{DMNS06},  the Laplacian mechanism has become the standard tool in differential privacy and has been used as the basic building block in a number of works on differential privacy analysis in other more complex problem settings, e.g., \cite{HLM12, MM09, Xiao11, Huang12, McSherry10, Li10, Barak07, DKMMN06, DL09, Roth10, LO11, Smith2011, CM08, continual, Ding11, Hardt2010, Geo12, Ka11, Mironov12bit, Sarathy2011, Xiao2011ireduct, Dankar12, Friedman10, zhang2012functional, lei2011differentially, wasserman2010, dwork2010pan, Guptadp2010, blum2011fast, hsu2012distributed, hsu2012dp, blocki2012johnson, hardt2012beyond, hardt2012private, gupta2012iterative, kasi13, karwa2011private, cormode2012differentially}. Given this near-routine use of the query-output independent adding of Laplacian noise,  the following two questions are natural:
\begin{itemize}
	\item Is  query-output independent perturbation optimal?
	\item Assume query-output independent perturbation,  is Lapacian noise distribution optimal?
\end{itemize}

In this work we answer the above two questions. Our main result is that given an $\e$-differential privacy constraint, under a general utility-maximization (equivalently, cost-minimization) model, for single real-valued query function (assuming local sensitivity is the same as global sensitivity),
\begin{itemize}
	\item adding query-output independent noise is indeed optimal (under a mild technical condition),
	\item the optimal noise distribution is {\em not} Laplacian distribution; instead, the optimal one has a {\em staircase-shaped} probability density function.
\end{itemize}

We also generalize the same result to the discrete setting where the query output is integer-valued and to more abstract settings.


% It is natural to ask the questions whether there exist other noise probability distributions which can outperform Laplacian distribution, and  what is the optimal probability distribution of the noise to preserve $\e$-differential privacy.

% We answer the above questions affirmatively in this work. We  study the fundamental limit of differential privacy and derive the optimal noise-adding mechanism to preserve $\e$-differential privacy under a very general utility-maximization (or equvialently, cost-minimization) framework. We show that in general Laplacian mechanism is not optimal, and the optimal noise probability distribution always has a staircase-shaped probability density function, which is specified by a parameter depending on the utility/cost functions.

\subsection{Problem Formulation}

We formulate a utility-maximization (cost-minimization) problem under the differential privacy constraint.

\subsubsection{Differential Privacy Constraint}
A general randomized releasing mechanism $\KM$ is a family of noise probability distributions indexed by  the query output (denoted by $t$), i.e.,
\begin{align}
 	\KM = \{\p_t : t \in \R \},
 \end{align}
and given dataset $D$, the mechanism $\KM$ will release the query output $t = q(D)$ corrupted by additive random noise with probability distribution $\p_t$:
\begin{align}
    \KM(D) = t + X_{t},
\end{align}
where $X_{t}$ is a random variable with probability distribution $\p_{t}$.


The differential privacy constraint \eqref{eqn:dpgeneral}    on $\KM$ is that for any $t_1,t_2 \in \R$ such that $|t_1 - t_2| \le \D $ (corresponding to the query outputs for two neighboring datasets) ,
\begin{align}
	\nm_{t_1} (S) \le e^{\e} \nm_{t_2}(S + t_1 - t_2), \forall \; \text{measurable set} \; S \subset \R,  \label{eqn:diffgeneralnoise1}
\end{align}
where for any $t \in \R$,  $S+t \, := \, \{s+t \, | \, s \in S\}$.

\subsubsection{Utility Model}

% We formulate a utility-maximization (cost-minimization) problem under the differential privacy constraint.
The utility model we use in this work is a very general one, which is also used in the works by Ghosh, Roughgarden, and Sundararajan \cite{Ghosh09}, Gupte and  Sundararajan \cite{minimax10}, and Brenner and Nissim \cite{Nissim10}.

Consider a cost function $\loss(\cdot): \R \to \R$, which is a function of the additive noise. Given additive noise $x$, the cost is $\loss(x)$. Given query output $t \in \R$, the additive noise is a random variable with probability distribution $\p_t$, and thus the expectation of the cost is
\begin{align}
	\int_{x\in \R} \loss(x) \p_t (dx).
\end{align}

The objective is to minimize the worst case cost among all possible query output $t \in \R$, i.e.,
\begin{align}
\text{minimize}\;  \sup_{t \in \R} \int_{x \in \R} \loss(x) \p_t(dx). \label{eqn:objective}
 \end{align}


\subsubsection{Optimization Problem}

Combining the differential privacy constraint \eqref{eqn:diffgeneralnoise1} and the objective function \eqref{eqn:objective}, we formulate a functional optimization problem:
\begin{align}
	\mathop{\text{minimize}}\limits_{ \{\p_t\}_{t \in \R}   } & \ \sup_{t \in \R} \int_{x \in \R} \loss(x) \p_t(dx) \label{eqn:objecinopt}\\
	\text{subject to} & \ \nm_{t_1} (S) \le e^{\e} \nm_{t_2}(S + t_1 - t_2), \forall \ \text{measurable set} \ S\subseteq \R, \ \forall |t_1 - t_2| \le \D.  \label{eqn:diffgeneralnoise}
\end{align}






%For more background and motivation of differential privacy, we refer the readers to the excellent survey \cite{DPsurvey} by Dwork.







\subsection{An Overview of Our Results}

\subsubsection{Adding Query-Output-Independent Noise is Optimal}

Our first result is  that  under a mild technical condition, adding query-output-independent noise is optimal, i.e., we can assume that $\p_t \equiv \p$ for all $t \in \R$ for some probability distribution $\p$.



For any positive integer $n$, and for any positive real number $T$, define
\begin{align}
 	\KM_{T,n} \triangleq \{\; \{\nm_t\}_{t \in \R}  \, |\, \{\nm_t\}_{t \in \R} \; \text{satisfies} \; \eqref{eqn:diffgeneralnoise}, \;  & \nm_t = \nm_{k \frac{T}{n}},   \text{for}\;   t \in [k\frac{T}{n}, (k+1)\frac{T}{n}), k \in \Z, \nonumber  \\
 & \text{and} \; \nm_{t+T} = \nm_{t}, \forall t \in \R    \}.
 \end{align}

\begin{theorem} \label{thm:maingeneral1}
 	Given any family of probability distribution $\{\nm_t\}_{t \in \R} \in  \cup_{T >0} \cup_{n \ge 1} \KM_{T,n}$,  there exists a probability distribution $\nm^*$ such that the family of probability distributions  $\{\p^*_t\}_{t \in \R}$ with $\p^*_t \equiv \p^*$  satisfies the differential privacy constraint \eqref{eqn:diffgeneralnoise} and
 	\begin{align}
 		  \sup_{t \in \R} \int_{x \in \R} \loss(x) \p^*_t(dx)     \le   \sup_{t \in \R} \int_{x \in \R} \loss(x) \p_t(dx) .
 	\end{align}	
 \end{theorem}

% \begin{theorem}[informal]
% 	Under a mild technical condition on the family of probability measure $\{\nm_t\}_{t \in \R}$, adding query-output-independent noise is optimal.
% \end{theorem}

%This result is  precisely stated in Theorem \ref{thm:maingeneral} in Section \ref{sec:optimality}.
Theorem \ref{thm:maingeneral1} states that if we assume the family of noise probability distributions is piecewise constant (the length of pieces can be arbitrarily small) over $t$, and periodic ( the period can be arbitrary) over $t$ , then in the optimal mechanism we can assume $\p_t$ does not dependent on $t$. We conjecture that the technical condition can be done away with.


\subsubsection{Optimal Noise Probability Distribution}

Due to Theorem \ref{thm:maingeneral1}, adding query-output-independent noise is optimal, and thus we only need to study what  the optimal noise probability distribution is. Let $\p$ denote the probability distribution of the noise added to the query output. Then the optimization problem \eqref{eqn:objecinopt} and \eqref{eqn:diffgeneralnoise} is reduced to
\begin{align}
	\mathop{\text{minimize}}\limits_{ \p} & \ \int_{x \in \R} \loss(x) \p (dx) \\
	\text{subject to} & \ \p(S) \le e^{\e} \p(S + d), \forall \ \text{measurable set} \ S\subseteq \R, \ \forall |d| \le \D.  \label{eqn:dpconstraintfinal}
\end{align}



Consider a staircase-shaped probability distribution with probability density function (p.d.f.) $f_{\gamma}(\cdot)$ defined as
\begin{align}
f_{\gamma}(x)  =
\begin{cases}
  	 a(\gamma) & x \in [0, \gamma \D) \\
 e^{-\e} a(\gamma) & x \in [\gamma \D,   \D) \\
  e^{-k\e} f_{\gamma}(x - k\D)  & x \in [ k \D,   (k+1)\D) \; \text{for} \; k \in \N \\
 f_{\gamma}(-x) & x<0
  \end{cases}\label{eqn:deffgamma}
\end{align}
where
\begin{align}
	a(\gamma) \triangleq \frac{ 1 - e^{-\e}}{2 \D (\gamma + e^{-\e}(1-\gamma))}
\end{align}
is a normalizing constant to make $\int_{x\in \R} f_{\gamma}(x) dx = 1$.


Our main result is
\begin{theorem}
	If the cost function $\loss(\cdot)$ is symmetric and increasing, and $\sup_{x \ge T} \frac{\loss(x+1)}{\loss(x)} < + \infty$ for some $T>0$, the optimal noise probability distribution has a staircase-shaped probability density function $f_{\gamma^*}(\cdot)$, where
	\begin{align}
		\gamma^* = \mathop{\arg \min} \limits_{\gamma \in [0,1] } \int_{x \in \R} \loss (x)  f_{\gamma}(x) dx .
	\end{align}
	
\end{theorem}

We plot the probability density functions of Laplace mechanism and staircase mechanism in Figure \ref{fig:probdf}. Figure \ref{fig:fgamma} in Section \ref{sec:result} gives a precise description of staircase mechanism.

The staircase mechanism is specified by three parameters: $\e$, $\D$, and $\gamma^*$ which is determined by $\e$ and the cost function $\loss(\cdot)$. For certain classes of cost functions, there are closed-form expressions for the optimal $\gamma^*$.



\begin{figure}[h]
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{fig_laplace.pdf}
\caption{ Laplace Mechanism }
\label{fig:compare1}
\end{subfigure}
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=0.8 \textwidth]{fig_stair.pdf}
\caption{ Staircase Mechanism}
\label{fig:compare2}
\end{subfigure}
\caption{Probability Density Functions of Laplacian Mechanism and Staircase Mechanism}
\label{fig:probdf}
\end{figure}



\subsubsection{Applications: Minimum Noise Magnitude and Noise Power}

We apply our main result Theorem \ref{thm:main} to two typical cost functions $\loss(x) = |x|$ and $\loss(x) = x^2$, which measure noise magnitude and noise power, respectively. We derive the closed-form expressions for the optimal parameters $\gamma^*$ for these two cost functions. Comparing the optimal performances with those of the Laplacian mechanism, we show that in the high privacy regime ($\e$ is small), the Laplacian mechanism is asymptotically optimal as $\e \to 0$;  in the low privacy regime ($\e$ is large), the minimum expectation of noise amplitude  and minimum noise power are $\Theta(\D e^{-\frac{\e}{2}})$ and $\Theta(\D^2 e^{-\frac{2\e}{3}})$ as $\e \to +\infty$, while  the expectation of noise amplitude and power using the Laplacian mechanism are $\frac{\D}{\e}$ and $\frac{2\D^2}{\e^2}$, respectively, where $\D$ is the sensitivity of the query function. We conclude that the gains are more pronounced in the low privacy regime.



\subsubsection{Extension to the Discrete Setting}

Since for many important practical applications query functions are integer-valued, we also derive the optimal differentially private mechanisms for answering a single integer-valued query function.
 We show that adding query-output independent noise is optimal under a mild technical condition, and the optimal noise probability distribution has a staircase-shaped probability mass function, which can be viewed as the discrete variant of the staircase mechanism in the continuous setting. 

 This result helps us directly compare our work and the existing works \cite{Ghosh09, minimax10} on integer-valued query functions. Our result shows that for integer-valued query function, the optimal noise probability mass function is also  staircase-shaped, and in the case the sensitivity $\D = 1$, the optimal probability mass function is reduced to the geometric distribution, which was derived in \cite{Ghosh09, minimax10}. Therefore, this result can be viewed as a generalization of \cite{Ghosh09, minimax10} in the discrete setting for query functions with arbitrary sensitivity.



%\subsubsection{Extensions to Discrete setting and  Abstract setting}

%We generalize our results on the optimal mechanism to preserve differential privacy to the discrete setting, where the query function is integer-valued. We show that adding query-output independent noise is optimal under a mild technical condition, and the optimal noise probability distribution has a staircase-shaped probability mass function, which can be viewed as the discrete variant of the staircase mechanism in the continuous setting.

%We show that the staircase mechanism can be also generalized to the abstract setting, where the query output can be in some abstract domain. The standard approach in this abstract setting is to use the exponential mechanism, introduced by McSherry and Talwar \cite{McSherry07}. We show that  replacing the exponential function by staircase function in the exponential mechanism can also preserve differential privacy, and in some special cases it is reduced to the staircase mechanism in the continuous setting.





\subsection{Connection to the Literature}\label{subsec:connection}

In this section, we discuss the relations of our results and some directly related works in the literature, and the implications of our results on  other works.

\subsubsection{Laplacian Mechanism vs Staircase Mechanism}



The Laplacian mechanism is specified by two parameters, $\e$ and the query function sensitivity $\D$. $\e$ and $\D$ completely characterize the  differential privacy constraint. On the other hand, the staircase mechanism is specified by three parameters, $\e$, $\D$, and $\gamma^*$ which is determined by $\e$ and the utility function/cost function. For certain classes of utility functions/cost  functions, there are closed-form expressions for the optimal $\gamma^*$.

From the two examples given in Section \ref{sec:application}, we can see that although the Laplacian mechanism is not strictly optimal, in the high privacy regime ($\e \to 0$), Laplacian mechanism is asymptotically optimal:
\begin{itemize}
	\item For the expectation of noise amplitude, the additive gap from the optimal values goes to 0 as $\e \to 0$,
	\item For noise power, the additive gap from the optimal values is upper bounded by a constant  as $\e \to 0$.
\end{itemize}
 However, in the low privacy regime ($\e \to +\infty$), the multiplicative gap from the optimal values can be arbitrarily large. We conclude that in the high privacy regime, the Laplacian mechanism is nearly optimal, while in the low privacy regime significant improvement can be achieved by using the staircase mechanism. We plot the multiplicative gain of staircase mechanism over Laplacian mechanism for expectation of noise amplitude and noise power in Figure  \ref{fig:comparison}, where $V_{\text{Optimal}}$ is the optimal (minimum) cost, which is achieved by staircase mechanism, and $V_{Lap}$ is the cost of Laplacian mechanism. We can see that for $\e \approx 10$, the staircase mechanism has about 15-fold and 23-fold improvement, with noise amplitude and power respectively.

Since the staircase mechanism is derived under the same problem setting as Laplacian mechanism, the staircase mechanism can be applied wherever Laplacian mechanism is used, and it performs strictly better than Laplacian mechanism (and significantly better in low privacy scenarios).

%When the query output has multiple components and the global sensitivity $\D$ is defined as the $\ell^1$-norm of difference between query outputs for two neighboring datasets, to preserve $\e$-differential privacy, Lapacian mechanism will add noise with Lapacian distribution with parameter $\frac{\D}{\e}$ to each component of query output independently, while if we simply add noise with staircase distribution to each component independently, the parameters of staircase distribution should be $(\frac{\e}{d}, \D, \gamma)$, where  $d$ is the number of query output components.

\begin{figure}[h]
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.1\textwidth]{fig1.pdf}
\caption{ $0 < \e \le 10 $}
\label{fig:compare1}
\end{subfigure}
\begin{subfigure}[b]{0.5\linewidth}
\centering
\includegraphics[width=1.1\textwidth]{fig2.pdf}
\caption{ $10 \le \e \le 20$}
\label{fig:compare2}
\end{subfigure}
\caption{Multiplicative Gain of the Staircase Mechanism over the Laplacian Mechanism. }
\label{fig:comparison}
\end{figure}




\subsubsection{Relation to Ghosh et. al. \cite{Ghosh09} }


Ghosh, Roughgarden, and Sundararajan  \cite{Ghosh09} show that for a single count query with sensitivity $\D = 1$, for a general class of utility functions, to minimize the expected cost under a Bayesian framework the optimal mechanism to preserve differential privacy is the geometric mechanism, which adds noise with geometric distribution.

We discuss the relations and differences between \cite{Ghosh09} and our work in the following: Both \cite{Ghosh09} and our work are similar in that,  given the query output, the cost function only depends on the additive noise magnitude, and is an increasing function of noise magnitude. On the other hand, there are two main differences:
\begin{itemize}

	\item \cite{Ghosh09}  works under a Bayesian setting, while ours is to minimize the worst case cost.

	\item \cite{Ghosh09} studies a count query where the query output is integer-valued, bounded and sensitivity is unity.  In our work,  we first study general real-valued query function where the query output can take any real value, and then generalize the result to discrete setting where query output is integer valued.  In both cases, the sensitivity of query functions can be arbitrary, not restricted to one.
\end{itemize}


\subsubsection{Relation to  Gupte and Sundararajan  \cite{minimax10}  }

  Gupte and Sundararajan \cite{minimax10} derive the optimal noise probability distributions for a single count query with sensitivity $\D = 1$ for minimax (risk-averse) users. Their model is the same as the one in \cite{Ghosh09} except that their objective function is to minimize the worst case cost, the same as our objective.  \cite{minimax10} shows that although there is no universally optimal solution to the minimax optimization problem in \cite{minimax10} for a general class of cost functions, each solution (corresponding to different cost functions) can be derived from the same geometric mechanism by randomly remapping.

  As in \cite{Ghosh09}, \cite{minimax10} assumes the query-output is bounded. Our result shows that when the query sensitivity is one, without any boundedness knowledge about the query-output, the optimal mechanism is to add random noise with geometric distribution to the query output.


\subsubsection{Relation to Brenner and Nissim  \cite{Nissim10}  }

While \cite{Ghosh09} shows that  for a single count query with sensitivity $\D = 1$, there is a universally optimal mechanism for a general class of utility functions  under a Bayesian framework, Brenner and Nissim  \cite{Nissim10}  show that for general query functions no universally optimal mechanisms exist. Indeed, this follows directly from our results:  under our optimization framework, the optimal mechanism is adding noise with staircase-shaped probability distribution which is specified by three parameters $\e, \D$ and $\gamma^*$, where in general $\gamma^*$ depends on the cost function.  Generally, for different cost functions, the optimal noise probability distributions have staircase-shaped probability density functions specified by different parameters.


\subsubsection{Relation to   Nissim, Raskhodnikova and Smith \cite{NRS07}  }

Nissim, Raskhodnikova and Smith \cite{NRS07} show that for certain nonlinear query functions, one can improve the accuracy by adding data-dependent noise calibrated to the smooth sensitivity of the query function, which is based on the local sensitivity of the query function. In our model, we use   the global sensitivity of the query function only, and assume that the local sensitivity is the same as the global sensitivity, which holds for a general class of query functions, e.g., count, sum.





\subsubsection{Relation to Hardt and Talwar  \cite{geometry}  }


Hardt and Talwar \cite{geometry} study the tradeoff between privacy and error for answering a set of linear queries over a histogram in a differentially private way. The  error is defined as the worst  expectation of the $\ell^2$-norm of the noise. The lower bound given in \cite{geometry} is $\Omega( \e^{-1} d\sqrt{d})$, where $d$ is the number of linear queries. An immediate consequence of our result is that for fixed d, when $\e \to +\infty$, an upper bound of $\Theta(e^{-\frac{\e}{3d}}d \sqrt{d})$ is achievable by adding independent staircase-shaped noise with parameter $\frac{\e}{d}$ to each component.


\subsubsection{Relation to Other Works}

There are many existing works on studying how to improve the accuracy for answering more complex queries under differential privacy, in which the basic building block is the standard Laplacian mechanism. For example, Hay et. al. \cite{Hay10} show that  one can improve the accuracy for a general class of histogram queries, by exploiting the consistency constraints on the query output, and Li et. al. \cite{Li10}  study how to optimize linear counting queries under differential privacy by carefully choosing the set of linear queries to be answered. In these works, the error is measured by the mean squared error of query output estimates, which corresponds to the variance of the noise added to the query output to preserve differential privacy. In terms of $\epsilon$, the error bound in these works scales linearly to $\frac{1}{\e^2}$, because of the use of Laplacian noise. If Laplacian distribution is replaced by staircase distribution in these works, one can improve the error bound to $\Theta(e^{-C\e})$ (for some constant $C$ which depends on the number of queries) when $\e \to +\infty$ (corresponding to the low privacy regime).




% In this work, we study the fundamental	tradeoff between privacy and utility in differential privacy. Specifically, given the differential privacy constraint, we derive  the optimal differentially private mechanism for  single real-valued query function under a very general utility-maximization (or cost-minimization) framework. The class of  noise probability distributions in the optimal mechanism has  {\em staircase-shaped} probability density functions which are symmetric (around the origin), monotonically decreasing and geometrically decaying. The staircase mechanism can be viewed as a {\em geometric mixture of uniform probability distributions}, providing a simple algorithmic description for the mechanism.  Furthermore, the staircase mechanism naturally generalizes to discrete query output settings as well as more abstract settings. We show that adding query-output independent noise with staircase distribution is optimal among all randomized mechanisms (subject to a mild technical condition) that preserve  differential privacy.

% We explicitly derive the optimal noise probability distributions with minimum expectation of noise amplitude and power.  Comparing the optimal performances with those of the Laplacian mechanism, we show that in the high privacy regime, Laplacian mechanism is asymptotically optimal;  in the low privacy regime, staircase mechanism signiﬁcantly outperforms Laplacian mechanism. We conclude that the gains are more pronounced in the low privacy regime.



\subsection{Organization}

The paper is organized as follows. We show the optimality of query-output independent perturbation in Section \ref{sec:optimality}, and present the optimal differentially private mechanism, staircase mechanism, in Section \ref{sec:result}. In Section \ref{sec:application}, we apply our main result to derive the optimal noise probability distribution with minimum expectation of noise amplitude and power, respectively, and  compare the performances with the Laplacian mechanism.  Section \ref{sec:gammaproperty} presents the asymptotic properties of $\gamma^*$ in the staircase mechanism for momentum cost functions, and suggests a heuristic choice of $\gamma$ that appears to work well for a wide class of cost functions. Section \ref{sec:discrete} generalizes the staircase mechanism for integer-valued query function in the discrete setting, and Section \ref{sec:abstractsetting} extends the staircase mechanism to the abstract setting. Section \ref{sec:conclusion} concludes this paper.





 %formulates the utility-maximization/cost-minimization under the differential privacy constraint  as a functional optimization problem. We present the solution (including an algorithmic representation) and our main result Theorem \ref{thm:main} in Section \ref{sec:result}, and the detailed proof is given in Appendix \ref{sec:proof}. In Section \ref{sec:application}, we apply our main result to derive the optimal noise probability distribution with minimum expectation of noise amplitude and power, respectively, and  compare the performances with the Laplacian mechanism.  Section \ref{sec:gammaproperty} presents the asymptotic properties of $\gamma^*$ in the staircase mechanism for momentum cost functions, and suggests a heuristic choice of $\gamma$ that appears to work well for a wide class of cost functions. Section \ref{sec:optimality} proves that adding query-output-independent noise with staircase distribution is optimal among all randomized differentially private mechanisms under a technical condition. Section \ref{sec:abstractsetting} extends the staircase mechanism to the abstract setting, and Section \ref{sec:discrete} generalizes the staircase mechanism for integer-valued query function in the discrete setting.


==> proof_backup.tex <==
%  In this work, we have a mild technical condition on the cost function, which essentially says the function can be unbounded and cannot increast too fast. Under the mild condition, we can guarantee that we can approximate any valid probability measure with piecewise constant p.d.f.
 


However, to the best knowledge of the authors, there is no work on discussing whether the Lapacian distribution is optimal or deriving the optimal noise distribution. This note answeres this question and shows that the Laplacian distribution is not optimal, and the optimal distribution has a p.d.f. which is a periodically decayiny step function. (move to introduction)


% Laplacian or Lapace.
% to make it more rigorous, argue that the measure for any point is zero. Then we can safely say we only need to consider right half of x-axis.


We assume the cost function $\loss(x)$ is symmetric and  monotone increasing for $x \ge 0$, i.e., $\loss(x) = \loss(-x)$, and $\loss(y) \le \loss(z) \forall 0 \le y \le z$.

In addition, we assume $\loss(x)$ satisfies a mild technical condition
\begin{property}
	Let $T$ be a positive integer such that $\loss(T) >0$. $\loss(x)$ satisfies 
	\begin{align}
	 	\sup_{x \ge T} \frac{\loss(x+1)}{\loss(x)} < + \infty. \label{eqn:propertyL}
	 \end{align} 
\end{property}



(first define the set of probability measures of finite cost)
Let $\p$ be a probability measure satisfying the differential privacy constraint and the cost is finite, i.e., 
\begin{align}
	V(\p) \triangleq \int_{x \in \R} \loss(x)  \p(dx) < + \infty.
\end{align}

We show that there exists a sequence of probability measures with symmetric piecewise constant probability density functions which satisfies the differential privacy constraint and have cost converging to $V(\p)$.

More precisely, we will prove that 
\begin{align}
	converge expresssion.
\end{align}

Since $\loss(x)$ satisfies \eqref{eqn:propertyL}, we can assume there exists a constant $B > 0$ such that 
\begin{align}
 	\loss(x+1) \le B \loss(x), \forall x \ge T.
 \end{align} 

Given $\delta >0$, since $V(\p)$ is finite, there exists integer $T^* >T$ such that
\begin{align}
	\int_{x \ge T^*} \loss(x)  \p(dx) < \frac{\delta}{B}.
\end{align}

For any integers $i \ge 1 $, $N \ge T^* $,
\begin{align}
	\int_{x \in [N,N+1)} \loss(x) \p^i (dx) & \le \p^i([N,N+1)) \loss(N+1) \\
	&= \p([N,N+1)) \loss(N+1) \\
	&\le \int_{x \in [N,N+1)} B \loss(x) \p  (dx).
\end{align}

Therefore,
\begin{align}
	\int_{x \in [T^*, +\infty)} \loss(x) \p^i (dx) &\le \int_{x \in [T^*, +\infty)} B \loss(x) \p (dx) \\
	&\le B \frac{\delta}{B} \\
	&= \delta.
\end{align}

For $x\in [0, T^*)$, $\loss(x)$ is a bounded function, and thus by the definition of  Riemann–Stieltjes integral, we have
\begin{align}
	\lim_{i \to \infty} \int_{x \in [0, T^*)} \loss(x) \p^i (dx) = \int_{x \in [0, T^*)} \loss(x) \p (dx).
\end{align}

So  there exists a sufficiently large integer  $i^*$ such that for all $i \ge i^*$
\begin{align}
	| \int_{x \in [0, T^*)} \loss(x) \p^{i} (dx) - \int_{x \in [0, T^*)} \loss(x) \p (dx)|  \le \delta.
\end{align}

Hence, for all $i \ge i^*$
\begin{align}
	& | \int_{x \in \R} \loss(x) \p^{i} (dx) - \int_{x \in \R} \loss(x) \p (dx) | \\
	=& 2 |(\int_{x \in [0, T^*)} \loss(x) \p^{i} (dx) - \int_{x \in [0, T^*)} \loss(x) \p(dx) + \int_{x \in [T^*, +\infty)} \loss(x) \p^{i} (dx)  - \int_{x \in [T^*, +\infty)} \loss(x) \p (dx)) | \\
	\le & 2 |(\int_{x \in [0, T^*)} \loss(x) \p^{i} (dx) - \int_{x \in [0, T^*)} \loss(x) \p(dx)|  + 2  \int_{x \in [T^*, +\infty)} \loss(x) \p^{i} (dx)  + 2 \int_{x \in [T^*, +\infty)} \loss(x) \p (dx) \\
	\le & 2 (\delta + \delta + \frac{\delta}{B}) \\
	\le &= (4+ \frac{2}{B}) \delta.
\end{align}

Therefore,
\begin{align}
	\lim_{i \to +\infty}    \int_{x \in \R } \loss(x) \p^i (dx) = \int_{x \in \R } \loss(x) \p (dx).
\end{align}














At the first glance, it is not clear whether the minimum variance exists. We will show the minimum variance indeeds exists and is achievable. For now, we   define the infimum of variances among all valid probability measures as
% change it soon!
\begin{align}
 	V^* \triangleq \inf_{\p \in \sP} \int x^2 d \p(x). \label{def:V}
 \end{align}

It is easy to argue that we only need to consider probability measures which are symmetric, i.e.,
\begin{align}
	\p(\s) = \p(-\s),
\end{align}
$\forall$ measurable set $\s \subset \R$. Indeed, suppose $\p \in \sP$, then we can define $\p_{sym}$ as
\begin{align}
	\p_{sym}(\s) \triangleq \frac{\p(\s) + \p(\s) }{2},
\end{align}
$\forall$ measurable set $\s \subset \R$.

It is easy to verify that $\p_{sym} \in \sP$ and it has the same variance as $\p$.

Therefore, if we define $\sP_{sym} \triangleq \{ \p_{sym} | \p \in \sP  \}$,
\begin{align}
 	D^* = 	\inf_{\p \in \sP_{sym}} \int x^2 d \p(x).
\end{align}


Next we state a lemma that for any $\p \in \sP_{sym}$, we can use a sequence of probability measures $\{ \p^i \}$ with piecewise constant probability density functions to approximate $\p$, while $\p^i \in \sP_{sym}$.

\begin{theorem}\label{thm:approx}
	Given $\p \in \sP_{sym}$. For any positive integer $i$, define a symmetric probability density function $f^i(x)$ as
	\begin{align}
		f^i(x) = \frac{ \p([k\frac{D}{i}, (k+1)\frac{D}{i} )}{\frac{D}{i}} ,  x\in [k\frac{D}{i}, (k+1)\frac{D}{i} ) for some nonnegative integer k, \\
		f^i(x) = f^i(-x), if x < 0.
	\end{align}
	Let $\p^i$ be the probability measure defined by
	\begin{align}
		\p^i(\s) \triangleq \int_{x\in \s} f(x) dx, \forall measurable set \s.
	\end{align}
	Then $\p^i \in \sP_{sym}$, and
	\begin{align}
		\lim_{i \to +\infty} \int_{x\in \R} x^2 \p^i(d x) = \int_{x \in \R} x^2 \p(dx)
= 2 \int_{x \ge 0} x^2 \p(dx).
	\end{align}
\end{theorem}

\begin{IEEEproof}
	Proof idea: first only need to consider integral over $[0, \infty)$ due to symmetry of the probability measure. Then split the interval into two parts, [0, ND) and [ND, +$\infty$]. Then use $\delta, \e$ argument. $\int_{x\in [0, ND) x^2 P(dx)}$ becomes  Riemann–Stieltjes integral. Then the division of bins is just one particular type of partitions. So it converges to the Riemann integral.

	Finally combine these two $\delta \e$ arguments, we prove the theorem.
\end{IEEEproof}


Define $\sP^{dis} \triangleq \{\p^i | \p \in \sP_{sym} , \forall positive integers i\}$, i.e., $\sP^{dis}$ is the set of probability measures satisfying differential privacy constraint and having symmetric piecewise constant probability density functions.

Due to Theorem \ref{thm:approx},
\begin{align}
	V^*  = \inf_{\p \in \sP^{dis}} \int x^2 d \p(x).
\end{align}
Therefore, to characterize $V^*$, we only need to study symmetric and piecewise consant probability density functions.


%% next argue that we only need to consider nondecreasing piecewise constant pdf

Next, we show that actually we only need to consider those symmetric piecewise constant probability density functions which are monotone decreasing when $x \ge 0$.

% this theorem prove that we only need to monotone decreasing pdf
\begin{theorem}\label{thm:monotone}
  Given a symmetric piecewise constant probability density function $f$ satisfying the differential privacy constraint and  $f(x) = a_k, x\in [k\frac{D}{i}, (k+1)\frac{D}{i} ) \forall x \ge 0$, i.e., $f$ is piecewise constant over intervals of length $\frac{D}{i}$. Then we can construct a new symmetric piecewise constant probability density function $g$ which satisfies differential privacy constraint and $g$ is monotone decreasing over $x \ge 0$, and
  \begin{align}
   	\int_{\R} x^2 g(x) dx \le \int_{\R} x^2 f(x) dx.
   \end{align}
\end{theorem}

\begin{proof}
Since $a_k \ge 0, \forall k \in \N$, and
\begin{align}
	\sum_{k=1}^{+\infty} a_k \frac{D}{i} = \frac{1}{2},
\end{align}
we conclude $\lim_{k \rightarrow +\infty} a_k = 0$.


% this must be true
Given the sequence $\{a_k\}$, construct a new monotone decreasing sequence $\{b_k\}$ and a bijective mapping $\pi: \N \rightarrow \N$ as follows
\begin{align}
	I_0 &= \argmax_{k \in \N} a_k, \label{eqn:max1}\\
	\pi (0) &= \min_{n \in I_0} n,  \text{i.e., smallest element in} I_0, \\
	b_0 &= a_{\pi(0)}, \\
	& \forall \text{integers}  m \ge 1, \\
	I_m &= \argmax_{k \in \N \backslash \{ \pi(j) |  j< m \}} a_k,  \label{eqn:max2} \\
	\pi (m) &= \min_{n \in I_m} n,  \text{i.e., smallest element in} I_m, \\
	b_m &= a_{\pi(m)}.
\end{align}

Since the sequence $\{a_k\}$ converges to 0,  the maximum of $a_k$ always exists in \eqref{eqn:max1} and \eqref{eqn:max2}. Therefore, $I_m$ is well defined for all $m \in \N$.

Note that since $\sum_{k=1}^{\infty} a_k \frac{D}{i} = 1$ and $\{b_k\}_{k \in \N}$ is simply a permutation of $\{a_k\}_{k \in \N}$, $\sum_{k=1}^{\infty} b_k \frac{D}{i} = \frac{1}{2}$.

Therefore, if we define a function $g$ as
$g(x) = b_k, x\in [k\frac{D}{i}, (k+1)\frac{D}{i} ) \forall x \ge 0$, and $g(x) = g(-x)$ for $x<0$, then $g$  is a valid probability density function, and
  \begin{align}
   	\int_{\R} x^2 g(x) dx \le \int_{\R} x^2 f(x) dx.
   \end{align}


Next, we need to prove that a probability measure with probability density function $g$   satisfies the differential privacy constraint. Since $\{b_k\}_{k \in \N}$ is a monotone noincreasing function, it is sufficient and necessary to prove that  for all $k \in \N$,
\begin{align}
		\frac{b_k}{b_{k+i}} \le e^{\e}.
\end{align}

To simplify notation, given $k$, we define
\begin{align}
	a^*(k) = \min_{ k \le j \le k+i} a_k,
\end{align}
i.e., $a^*(k)$ denotes the smallest number of  $\{ a_{k}, a_{k+1}, \dots, a_{k+i} \}$.


First, when $k = 0$, it is easy to prove that $\frac{b_0}{b_{i}} \le e^{\e}$. Indeed, recall that $b_0 = a_{\pi(0)}$ and consider the $i+1$ consecutive numbers $\{a_{\pi(0)}, a_{\pi(0)+1}, \dots, a_{\pi(0)+i} \}$ in the original sequence $\{a_k\}_{k \in \N}$.    Then  $a^*(0) \le b_i$, since $b_i$ is the $(i+1)$th largest number in the sequence $\{a_k\}_{k \in \N}$. Therefore,
\begin{align}
	\frac{b_0}{b_{i}}  = \frac{a_{\pi(0)}}{b_{i}} \le  \frac{a_{\pi(0)}}{a^*(0)} \le e^{\e}.
\end{align}


For $k = 1$, $b_1 = a_{\pi(1)}$ and consider the $i+1$ consecutive numbers $\{a_{\pi(1)}, a_{\pi(1)+1}, \dots, a_{\pi(1)+i} \}$. If $\pi(0) \notin [\pi(1), \pi(1)+i]$, then $a^*(\pi(1)) \le b_{i+1}$, and thus
\begin{align}
	\frac{b_1}{b_{i+1}}  = \frac{a_{\pi(1)}}{b_{1+i}} \le  \frac{a_{\pi(1)}}{a^*(\pi(1))} \le e^{\e}.
\end{align}
If $\pi(0) \in [\pi(1), \pi(1)+i]$, then $a^*(\pi(0)) \le b_{i+1}$ and $\frac{a_{\pi(0)}}{a^*(\pi(0))} \le e^{\e}$. Therefore,
\begin{align}
	\frac{b_1}{b_{i+1}}  \le \frac{b_0}{b_{1+i}} \le  \frac{b_0}{a^*(\pi(0))} \le e^{\e}.
\end{align}
Hence, $\frac{b_k}{b_{k+i}} \le e^{\e}$ holds for $k = 1$.

In general, given $k$,  we prove $\frac{b_k}{b_{k+i}} \le e^{\e}$ as follows. First, if $\pi_{j} \notin [\pi(k), \pi(k)+i], \forall j <k$, then $a^*{\pi(k)} \le b_{k+i}$, and hence
\begin{align}
	\frac{b_k}{b_{i+k}}  = \frac{a_{\pi(k)}}{b_{i+k}} \le  \frac{a_{\pi(k)}}{a^*(\pi(k))} \le e^{\e}.
\end{align}
If there exists $j < k$ and $\pi_{j} \in [\pi(k)+1, \pi(k)+i]$, we use the following algorithm to compute a number $j^*$ such that $ j^* < k $ and $\pi_{j} \notin [\pi(j^*)+1, \pi(j^*)+i], \forall j<k$.

\begin{algorithm}
\begin{algorithmic}
\State $j^*  \gets k$
\While{ there exists some $j <k $ and $\pi_{j} \in [\pi(j^*)+1, \pi(j^*)+i]$}
	\State $j^*  \gets j$
\EndWhile
\State Output $j^*$
\end{algorithmic}
\end{algorithm}

It is easy to show that the   loop in the algorithm will  terminate after at most $k$ steps.

After finding $j^*$, we have $j^* < k$, and $a^*(\pi(j^*)) \le b_{k+i}$. Therefore
\begin{align}
 	\frac{b_k}{b_{i+k}}  \le \frac{a_{\pi(j^*)}}{b_{i+k}} \le  \frac{a_{\pi(j^*)}}{a^*(\pi(j^*))} \le e^{\e}.
 \end{align}

 So $\frac{b_k}{b_{k+i}} \le e^{\e} $  holds for all $k \in \N$.

% summary: Therefore
\end{proof}



Therefore, if we define
\begin{align}
	\sP^{m} \triangleq \{ \p | \p \in \sP^{dis}, \text{and} \p \text{has a monotone decreasing p.d.f when $x \ge 0$}  \},
\end{align}
i.e., the set of symmetric probability measures with monotone nonincreasing piecewise constant p.d.f when $x \ge 0$, then
due to Theorem \ref{thm:monotone}
\begin{align}
	V^* = \inf_{\p \in \sP^{m}}   \int x^2 d \p(x)  .
\end{align}


Next, we argue that among all symmetric piecewise constant pdf, we only need to consider those which are periodically decaying.

More precisely, given positive integer $i$, define $\p_i$ as the set of probability measures with symmetric and piecewise constant p.d.f with period $\frac{D}{i}$, and the density sequence $\{a_0,a_1,\dots,a_n,\dots \}$ satisfies that
\begin{align}
 	\frac{a_k}{a_{k+i}} = e^{\e}, \forall k \ge 0.
 \end{align}



We claim that
\begin{theorem}
\begin{align}
		V^* = \inf_{ \p  in \cup_{i=1}^{\infty} \p_i}  \int x^2 d \p(x).
\end{align}

\end{theorem}

\begin{IEEEproof}
	Due to Theorem \ref{thm:monotone}, we only need to consider those measures with symmetric and monotone decreasing piecewise constant pdf.

	We will show that for any nonnegative integer $i$, among the probability measures with symmetric and monotone decreasing piecewise constant pdf with period $\frac{D}{i}$, we only need to consider those with exponentially decaying coefficients, i.e.,
	\begin{align}
 		\frac{a_k}{a_{k+i}} = e^{\e}, \forall k \ge 0,
 	\end{align}
 	to minimize the noise variance.

 	First we show $\frac{a_{0}}{a_{i}} = e^{\e}$. Suppose $\frac{a_{0}}{a_{i}} < e^{\e}$. Then we can define a new sequence $\{b_0,b_1,\dots,b_n,\dots\}$ by scaling up $a_0$ and scaling down ${a_1,a_2,\dots}$. More precisely, let  $\delta = \frac{i}{2D ( (\frac{i}{2D}-a_0)e^{-\e}\frac{a_0}{a_i} + a_0  )} - 1 >0$, and set
 	\begin{align}
 	 	b_0 = a_0 (1 + \delta), \\
 	 	b_k = a_k ( 1 - \delta'), \forall k \ge 1,
 	 \end{align}
 	 where $ \delta' \triangleq \frac{a_0 \delta}{ \frac{i}{2D} - a_0} >0$,
 	 and we have chosen $\delta$ such that $\frac{b_0}{b_i} = \frac{a_0}{a_k} \frac{\frac{i}{2D} - a_0}{ \frac{i}{2D(1+\delta)} - a_0} = e^{\e}$.

 	It is easy to see the sequence $\{b_i\}$ correspond to a valid probability density function and it also satisfies the differential privacy constraint, i.e.,
 	\begin{align}
 		\frac{b_k}{b_{k+i}} \le e^{\e}, \forall k \ge 0.
 	\end{align}

 	Next we show that $\{b_k\}$ gives a smaller variance than $\{a_k\}$. % make this satement more precise

 	It is easy to compute the variance of probability measure corresponding to $\{a_k\}$, which is
 	\begin{align}
 		V_a = 2\frac{D}{i} ( a_0 \int_{0}^{\frac{D}{i}} x^2 dx  + \sum_{k=1}^{\infty} a_k \int_{k\frac{D}{i}}^{(k+1)\frac{D}{i}}    x^2 dx ).
 	\end{align}

 	Similarly, the variance of probability measure corresponding to $\{b_k\}$ is
 	\begin{align}
 		V_b &= V_a + 2\frac{D}{i}  (a_0 \delta \int_{0}^{\frac{D}{i}} x^2 dx  -  \delta' \sum_{k=1}^{\infty} a_k \int_{k\frac{D}{i}}^{(k+1)\frac{D}{i}}    x^2 dx) \\
 		&= V_a +  2\frac{D}{i} \frac{a_0 \delta}{ \frac{i}{2D} - a_0  } ( \sum_{k=1}^{\infty} a_k \int_{0}^{\frac{D}{i}} x^2 dx - \sum_{k=1}^{\infty} a_k \int_{k\frac{D}{i}}^{(k+1)\frac{D}{i}}    x^2 dx ) \\
 		&= V_a +  2\frac{D}{i} \frac{a_0 \delta}{ \frac{i}{2D} - a_0  } ( \sum_{k=1}^{\infty} a_k (  \int_{0}^{\frac{D}{i}} x^2 dx -     \int_{k\frac{D}{i}}^{(k+1)\frac{D}{i}}    x^2 dx     ) ) \\
 		&< V_a.
 	\end{align}


 	Therefore, for fixed nonnegative integer $i$, we only need to consider those probability measures with $\frac{a_0}{a_i} = e^{\e}$.

 	Next, we argue that among those probability measures with $\frac{a_0}{a_i} = e^{\e}$, we only need to consider thoses probability measures which also satisfies $\frac{a_1}{a_{i+1}} = e^{\e}$. Suppose, given montone decreasing p.d.f sequence $\{a_k\}$ which satisfies $\frac{a_0}{a_i} = e^{\e}$, and $\frac{a_0}{a_i} < e^{\e}$, then we can construct a new sequence $\{b_k\}$  satisfying
 	\begin{align}
 	 	\frac{b_0}{b_i} &= e^{\e}, \\
 	 	\frac{b_1}{b_{i+1}} &= e^{\e},
 	 \end{align}
	and having a smaller variance.

	First, it is easy to see $a_1$ is strictly  less than $a_0$, since if $a_0 = a_1$, then $\frac{a_1}{a_{i+1}} = \frac{a_0}{a_{i+1}} \ge \frac{a_0}{a_i} = e^{\e}$. Then we construct a new sequence by increasing $a_1$ and decreasing $a_{i+1}$. More precisely, we define a new sequence $\{a^{(1)}_k\}$ as
	\begin{align}
		a^{1}_k &= a_k, \forall k \neq 1, k \neq i+1, \\
		a^{1}_1 &= a_1 + \delta, \\
		a^{1}_{i+1} &= a_{i+1} - \delta,
	\end{align}
	where $\delta = \frac{e^{\e}a_{i+1} - a_1}{1 + e^{\e}}$ and thus $\frac{a^{1}_1}{a^{1}_{i+1}} = e^{\e}$.

	It is easy to verify that $\{a^{(1)}_k\}$ is a valid p.d.f sequence and it satisfies the differential privacy constraint. Moreover, it has a smaller variance than the original sequence $\{a_k\}$. Therefore, we only need to consider those probability measures with sequences $\{a_k\}$ satisfying $\frac{a_0}{a_i} = e^{\e}$, and $\frac{a_0}{a_i} = e^{\e}$.



	% we can make this argument more rigorous. Basically, I think we need to show that the new sequence must also be monotone decreasing. If $a^{1}_{i+1} \ge a^{1}_{i+1}$, then $\{a^{(1)}_k\}$ is a montone decreasing sequence, we are done. Suppose $a^{1}_{i+1} < a^{1}_{i+1}$, then we can rearrange the parts a_k for k>i+1 in decreasing order. And use the same delta technique. Since sum of a_k is finite. There are only finite number of k such that a_k is larger than a^(1)_{i+1}. So this change will terminate in finite number of steps. Therefore eventually we will get a monoton decreasing sequence.


	Use the same argument, we can show that we only need to consider those probability measures with sequences $\{a_k\}$ satisfying
	\begin{align}
		\frac{a_k}{a_{i+k}} &= e^{\e}, \forall k \ge 0.
	\end{align}


 % basically, if a{k} / a{k+i} < e^{\e}, then we can increase a_k and decrease a_{k+i}. We donot need to worry about whether a_k would be larger than a_{k-1}. THis won't happen. because if a{k-1}/a{k-1+i} = e^{\e}.



 	Therefore,
 	\begin{align}
		V^* = \inf_{ \p  \in \cup_{i=1}^{\infty} \p_i}  \int x^2 d \p(x).
	\end{align}

% introduce notation P_i to denote the probability measures with monotone decreasing and periodically decaying picewise constant p.d.f., and the number of bins in each period $[0,\D]$ is $i$.


\end{IEEEproof}



The above argument allows us only need to consider  probability measures with symmetric monotone decreasing and periodically decaying piecewise linear constant probability density function. Due to the properties of symmetry and periodically decaying, for  this class of probability measures the probability density funciton is completely determined by the p.d.f. over the interval $[0, \D)$.

Next, we study what the optimal p.d.f. should be over the interval $[0,\D)$. It turns out that the optimal p.d.f. over the interval $[0,\D)$ is a step function.

We use three steps to prove this claim. XXXX

\begin{lemma}\label{lem:ratio}
	Consider a probability measure $\p_a \in \p_i$, with density sequence $\{a_0,a_1,\dots, a_n,\dots\}$, and $\frac{a_0}{a_{i-1}} < e^{\e}$. Then there exists a probability measure $\p_b \in \p_i$ with   density sequence $\{b_0,b_1,\dots, b_n,\dots\}$, such that  $\frac{b_0}{b_{i-1}} = e^{\e}$, and
	\begin{align}
		\int_{-\infty}^{+\infty} \loss (x) d \p_b(x) \le  \int_{-\infty}^{+\infty} \loss (x) d \p_a(x).
	\end{align}
\end{lemma}

\begin{IEEEproof}
	
	For each $ 0 \le k \le (i-1)$, define
	\begin{align}
		w_k \triangleq \sum_{j=0}^{+\infty} e^{-j\e} \int_{(j + \frac{k}{i})\D  }^{(j + \frac{k+1}{i})\D} \loss (x) d x.  \label{eqn:sumw}
	\end{align}

Since XXXXX condition on loss function, the sum of series in \eqref{eqn:sumw} exists, and thus $w_k$ is well defined for all $ 0 \le k \le (i-1)$. In addition, it is easy to see
\begin{align}
	w_0 \le w_1 \le w_2 \le \cdots \le w_{i-1},
\end{align}
since $\loss (x)$ is a monotone increasing function when $x \ge 0 $.

Then
\begin{align}
	\int_{-\infty}^{+\infty} \loss (x) d \p_a(x) = 2 \sum_{k=0}^{i-1} w_k a_k.
\end{align}

Since $\frac{a_0}{a_{i-1}} < e^{\e}$, we can scale $a_0$ up and scale $a_1,\dots,a_{i-1}$ down to derive a new valid probability density function with smaller penalty. More precisely, define a new probability measure $\p_b \in \p_i$ with   density sequence $\{b_0,b_1,\dots, b_n,\dots\}$ via
\begin{align}
	b_0 &\triangleq \gamma a_0, \\
	b_k &\triangleq \gamma' a_k, \forall 1 \le k \le i-1,
\end{align}
for some $\gamma >1 $ and $\gamma' <1$ such that
\begin{align}
 	\frac{b_0}{b_{i-1}} = e^{\e}.
 \end{align}

To make   $\{b_0,b_1,\dots, b_n,\dots\}$ be a valid density sequence, i.e., to make the integral of the corresponding p.d.f. over $\R$ be 1, we have
\begin{align}
	\sum_{k=0}^{i-1} b_k = \sum_{k=0}^{i-1} a_k = \frac{1-e^{-\e}}{2} \frac{i}{\D}.
\end{align}

Define $t \triangleq \frac{1-e^{-\e}}{2} \frac{i}{\D}$, then we have two linear equations on $\gamma$ and $\gamma'$:
\begin{align}
	\gamma a_0 &= e^{\e} \gamma' \label{eqn:g1} \\
	\gamma a_0 + \gamma' (t - a_0) &= t. \label{eqn:g2}
\end{align}

From \eqref{eqn:g1} and  \eqref{eqn:g2}, we can easily get
\begin{align}
	\gamma &= \frac{e^{\e} t a_{i-1}}{a_0 (t-a_0+e^{\e}a_{i-1})}  >1 \\
	\gamma' &= \frac{t}{ t-a_0+e^{\e}a_{i-1}}  <1.
\end{align}

Then we can easily verify that the cost of $\p_b$ is no bigger than the cost of $\p_a$. Indeed,
\begin{align}
	& \int_{-\infty}^{+\infty} \loss (x) d \p_a(x) - \int_{-\infty}^{+\infty} \loss (x) d \p_b(x)  \\
	= & 2 \sum_{k=0}^{i-1} w_k a_k -  2 \sum_{k=0}^{i-1} w_k b_k \\
	= & 2 ((1 - \gamma) w_0 a_0  + (1 -  \gamma') \sum_{k=1}^{i-1} w_k a_k   ) \\
	\ge & 2 ((1 - \gamma) w_0 a_0  + (1 -  \gamma') \sum_{k=1}^{i-1} w_0 a_k   ) \\
	= & 2 ((1 - \gamma) w_0 a_0  + (1 -  \gamma')   w_0 (t  - a_0 )  ) \\
	= & 2 w_0 (a_0 - \frac{a_{i-1}e^{\e}t}{t - a_0 + e^{\e}a_{i-1}} + (t - a_0)\frac{-a_0 + e^{\e}a_{i-1}}{t - a_0 + e^{\e}a_{i-1}}            )  \\
	= & 0.
\end{align}


This completes the proof.

\end{IEEEproof}


Therefore, due to Lemma \ref{lem:ratio}, for all integer $i \ge 2$, we only need to consider probability measures $\p \in \p_i$ with density sequence  $\{a_0,a_1,\dots, a_n,\dots\}$ satisfying $\frac{a_0}{a_{i-1}} = e^{\e}$.

More precisely, define
\begin{align}
	\pc_i = \{ \p \in \pb_i | \p \text{has density sequence}  \{a_0,a_1,\dots, a_n,\dots\} \text{with}   \frac{a_0}{a_{i-1}} = e^{\e}  \}.
\end{align}
Then due to Lemma \ref{lem:ratio},
\begin{lemma}
	\begin{align}
		V^* = \inf_{\p \in \cup_{i=2}^{\infty}\pc_i}  \int_{-\infty}^{+\infty} \loss (x) d \p(x) .
	\end{align}

\end{lemma}


%% make it more precise
Next, we argue that  for each probability measures $\p \in \pc_i$  ($i \ge 3$) with density sequence $\{a_0,a_1,\dots, a_n,\dots\}$ , we can assume that there exists an integer $1 \le k \le (i-2)$, such that
\begin{align}
	a_j &= a_0, \forall 0 \le j <k, \label{eqn:property1} \\
	a_j &= a_{i-1}, \forall k< j <i. \label{eqn:property2}
\end{align}

More precisely,
\begin{lemma}\label{lem:binary}
		Consider a probability measure $\p_a \in \pc_i$ ($i \ge 3$) with density sequence $\{a_0,a_1,\dots, a_n,\dots\}$. Then there exists a probability measure $\p_b \in \pc_i$ with density sequence $\{b_0,b_1,\dots, b_n,\dots\}$, such that there exists integer $1 \le k \le (i-2)$ with
		\begin{align}
		b_j &= a_0, \forall 0 \le j <k, \\
		b_j &= a_{i-1}, \forall k< j <i,
		\end{align}
and
	\begin{align}
		\int_{-\infty}^{+\infty} \loss (x) d \p_b(x) \le  \int_{-\infty}^{+\infty} \loss (x) d \p_a(x).
	\end{align}
\end{lemma}

\begin{IEEEproof}
	If there exists integer $1 \le k \le (i-2)$ such that
		\begin{align}
		a_j &= a_0, \forall 0 \le j <k, \\
		a_j &= a_{i-1}, \forall k< j <i,
		\end{align}
then we can set $\p_b = \p_a$.

Otherwise, let $k_1$ be the smallest integer in $\{ 0,1,2,\dots, i-1\}$ such that
\begin{align}
	a_{k_1} \neq a_0,
\end{align}
and let $k_2$ be the biggest integer in $\{ 0,1,2,\dots, i-1\}$ such that
\begin{align}
	a_{k_2} \neq a_{i-1}.
\end{align}

It is easy to see that $k_1 \neq k_2$. Then we can increase $a_{k_1}$ and decrease $a_{k_2}$ simultaneouly by the same amount to derive a new probability measure $\p_a^{(1)} \in \pc_i$ with smaller cost. Indeed, if
\begin{align}
	a_0 - a_{k_1} \leq a_{k_2} - a_{i-1},
\end{align}
then consider a probability measure $\p_a^{(1)} \in \pc_i$ with  density sequence  $\{ a^{(1)}_0, a^{(1)}_1, \dots, a^{(1)}_{i-1} ,\dots \}$ defined as
\begin{align}
	a^{(1)}_j &= a_0, \forall 0 \le j \le k_1, \\
	a^{(1)}_j &= a_j, \forall k_1 < j \le k_2-1, \\
	a^{(1)}_{k_2} &= a_{k_2} - (a_0 - a_{k_1}),   \\
	a^{(1)}_j &= a_j, \forall k_2 < j \le i-1.
\end{align}

It is easy to see the cost of $\p_a^{(1)} $ is no bigger than the cost of $\p_a$ via
\begin{align}
 	& \int_{-\infty}^{+\infty} \loss (x) d \p_a^{(1)}(x) - \int_{-\infty}^{+\infty} \loss (x) d \p_a(x) \\
 	= & 2 (w_{k_1} a^{(1)}_{k_1} + w_{k_2} a^{(1)}_{k_2} )   - 2 ( w_{k_1} a_{k_1} + w_{k_2} a_{k_2}) \\
 	= & 2  w_{k_1} (a_0 - a_{k_1}) + 2 w_{k_2} ( a_{k_2} - (a_0 - a_{k_1}) - a_{k_2}  ) \\
 	= &  2  (a_0 - a_{k_1}) ( w_{k_1}  - w_{k_2}) \\
 	\le & 0 ,
 \end{align}
 where $w_i$ is defined in \eqref{eqn:sumw}.

 Therefore, continue in this way, and finally we will obtain a probability measure $\p_b \in \pc_i$ with density sequence $\{b_0,b_1,\dots, b_n,\dots\}$, such that there exists integer $1 \le k \le (i-2)$ with
		\begin{align}
		b_j &= a_0, \forall 0 \le j <k, \\
		b_j &= a_{i-1}, \forall k< j <i,
		\end{align}
and
	\begin{align}
		\int_{-\infty}^{+\infty} \loss (x) d \p_b(x) \le  \int_{-\infty}^{+\infty} \loss (x) d \p_a(x).
	\end{align}

This completes the proof.

\end{IEEEproof}



%%%%%%%%%%%%%%%%%%%%%%% next step %%%%%%%%%%%%%%%%%%%%
Define
\begin{align}
	\pd_i = \{ \p \in \pc_i \ |\ \p \text{has density sequence satisfying \eqref{eqn:property1} and \eqref{eqn:property2} for some $k$}  \}.
\end{align}

Therefore, due to Lemma \ref{lem:binary},
\begin{lemma}\label{lem:stepfunc}
	\begin{align}
		V^* = \inf_{\p \in \cup_{i=3}^{\infty}\pd_i}  \int_{-\infty}^{+\infty} \loss (x) d \p(x) .
	\end{align}
\end{lemma}



Given $\gamma \in [0,1]$, define
\begin{align}
	a(\gamma) \triangleq \frac{ 1 - e^{-\e}}{2 \D (\gamma + e^{-\e}(1-\gamma))}.
\end{align}

Consider a class of probability distribution with symmetric and  staircase-shaped probability density function. Fix $\gamma \in [0,1]$, then define $\p^{\gamma}$ as the probability distribution with probability density function $f_{\gamma}(\cdot)$ defined as
\begin{align}
f_{\gamma}(x) &=  a(\gamma), x \in [0, \gamma \D) \\
f_{\gamma}(x) &= e^{-\e} a(\gamma), x \in [\gamma \D,   \D) \\
f_{\gamma}(x) &= e^{-k\e} f_{\gamma}(x - k\D) , x \in [ k \D,   (k+1)\D) \text{for} k \in \N \\
f_{\gamma}(x) &= f_{\gamma}(-x), x<0.
\end{align}

It is easy to verify that $f_{\gamma}(\cdot)$ is a valid probability density function and $\p^{\gamma}$ satisfies the differential privacy constraint.

Our main result is
\begin{theorem}\label{thm:main}
\begin{align}
	V^* = \inf_{\gamma \in [0,1]}  \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma}(x) .
\end{align}
\end{theorem}

\begin{IEEEproof}
	Due to the definition of $V^*$ in \eqref{def:V}, we have
	\begin{align}
		V^* \le \inf_{\gamma \in [0,1]}  \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma}(x).
	\end{align}

	We prove the reverse direction in the following.

	We first prove that for any $\p \in \pd_i$ ( $i \ge 3$), there exists $\gamma \in [0,1]$ such that
	\begin{align}
		\int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma}(x) \le \int_{-\infty}^{+\infty} \loss (x) d \p(x).
	\end{align}

	Consider the density sequence $\{a_0,a_1,\dots, a_n,\dots\}$ of $\p$. Since $\p \in \pd_i$, there exists an integer $ 0 \le k \le i-2 $ such that
	\begin{align}
		a_j = a_0, \forall 0 \le j< k, \\
		a_j = a_0 e^{-\e}, \forall k < j \le i-1.
	\end{align}

	Let
	\begin{align}
		\gamma^* \triangleq \frac{\frac{1-e^{-\e}}{2\D} - a_0 e^{-\e}}{a_0(1-e^{-\e})} \in [0,1].
	\end{align}
	Then $a(\gamma^*) = a_0$.

	It is easy to verify that  % prove it by contradiction
	\begin{align}
		k \frac{\D}{i} \le \gamma^* \D \le (k+1) \frac{\D}{i}.
	\end{align}

	The probability density functions of $\p$ and $\p^{\gamma^*}$ are the same when $ x \in [0, \frac{k}{i}\D) \cup [\frac{k+1}{i}\D, \D)$. Since the integral of probability density functions over $[0, \D)$ is  $\frac{1 - e^{-\e}}{2}$, we have
	\begin{align}
		a_k \frac{\D}{i} = a_0 (\gamma^* - \frac{k}{i}) \D + e^{-\e}a_0 ( \frac{k+1}{i} - \gamma^*)\D.
	\end{align}

	Define $\beta \triangleq i (  \gamma^* - \frac{k}{i} ) \in [0,1]$. Then
	\begin{align}
		a_k = \beta a_0 + (1 - \beta) e^{-\e}a_0.
	\end{align}

    Define 
    \begin{align}
		w_k^{(1)} &\triangleq \sum_{j=0}^{+\infty} e^{-j\e} \int_{(j + \frac{k}{i})\D  }^{(j + \gamma^*) \D} \loss (x) d x,  \label{eqn:sumw1} \\
    w_k^{(2)} &\triangleq \sum_{j=0}^{+\infty} e^{-j\e} \int_{(j +  \gamma^*) \D    }^{(j + \frac{k+1}{i} )\D} \loss (x) d x,  \label{eqn:sumw2}.
	\end{align}
    Note that $w_k = w_k^{(1)} + w_k^{(2)}$. Since $\loss(x)$ is a monotone increasing function when $x \ge 0$, we have
    \begin{align}
    	\frac{w_k^{(2)}}{w_k^{(1)}} \ge \frac{(j + \frac{k+1}{i} )\D -  (j +  \gamma^*) \D  }{(j + \gamma^*) \D - (j + \frac{k}{i})\D} = \frac{\frac{k+1}{i} - \gamma^*}{\gamma^* - \frac{k}{i} }.
    \end{align}

	Therefore,
	\begin{align}
 	& \int_{-\infty}^{+\infty} \loss (x) d \p(x) - \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma^*}(x) \\
 	= & 2 w_{k} a_{k}  - 2 ( w_k^{(1)}  a_0 +  w_k^{(2)}  a_0 e^{-\e}) \\
 	= & 2  (w_k^{(1)} + w_k^{(2)}) a_k - 2 ( w_k^{(1)}  a_0 +  w_k^{(2)}  a_0 e^{-\e})  \\
 	= &  2  ( a_k - a_0 e^{-\e} )w_k^{(2)} -  2  (a_0 - a_k ) w_k^{(1)} .
 	\end{align}

 	Since 
 	\begin{align}
 		\frac{a_k - a_0 e^{-\e} }{a_0 - a_k} &= \frac{ \beta (a_0 - a_0 e^{-\e})}{(1-\beta) (a_0 - a_0 e^{-\e}) } \\
 		&= \frac{\beta}{1 - \beta} \\
 		&= \frac{\gamma^* - \frac{k}{i}}{\frac{k+1}{i} - \gamma^*} \\ 
 		&\ge \frac{w_k^{(1)}}{w_k^{(2)}},
 	\end{align}
 	we have
 	\begin{align}
 		& \int_{-\infty}^{+\infty} \loss (x) d \p(x) - \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma^*}(x) \\
 		= &  2  ( a_k - a_0 e^{-\e} )w_k^{(2)} -  2  (a_0 - a_k ) w_k^{(1)} \\
 		\ge & 0.
 	\end{align}

 	Therefore,
 	\begin{align}
 		V^* &= \inf_{\p \in \cup_{i=3}^{\infty}\pd_i}  \int_{-\infty}^{+\infty} \loss (x) d \p(x) \\
 		& \ge \inf_{\gamma \in [0,1]}  \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma}(x) .
 	\end{align}

 	We conclude
 	\begin{align}
 		V^*  = \inf_{\gamma \in [0,1]}  \int_{-\infty}^{+\infty} \loss (x) d \p^{\gamma}(x) .
 	\end{align}

\end{IEEEproof}


% Next, we only need to consider those monotone decreasing XXX

% 1) first argue, in for each discrete pdf. $a_i/a_0 = e^{\e}$

% 2) Then argue, there is only at most one segment which is not equal to $a_i$ or $a_0$

% 3) Given a_0, define the optimal pdf with starting value a_0, then
% show that for any discrete pdf start with a_0, the loss value is no less than the optimal one.
% 	This can divide into two steps
% 	  a) show that r^* is lies in the segment where not a_0, not a_i
% 	  b) then show that the variance is larger

% 	  both steps are very easy to prove

% Then we can conclude the optimal noise strucutre is found, and to get the optimal noise distribution we only need to solve an optimization problem.
















==> winter_break.tex <==

In the winter break, we plan to solve the following four problems

1) Prove the optimality of the staircase mechanism among all possible mechanisms

The hard part is to define the average of uncountable probability measures 

It can be shown that the cost is invariant of translation (i.e., shift) of the family of probability measures. And any linear convex combination of probability meausures satisfying DP is still a valid probability measure.

Due to the above two properties, if we put two  constraints on the family of probability measures:
1) piecewise constant, i.e., \mu_x is independent of x for x in each interval, the length of the interval can be arbitrarily small.  
2) peridoic, i.e, \mu_x = \mu_x (kT), where k can be arbitrarily large.  

Then it is easy to prove that in the optimal noise probability distribution, we can assume \mu_x is independent of x over the real line.






2) Prove the optimal mechanism in the finite range case

This seems impossible. But for discrete case with D >=2, maybe we can get some results.









3) Extend the result to abstract setting as in the paper of exponential mechanism


One way is to use score function to partition the real line, as done in Talwar's paper.

The other way is to define a metric space in the original dataset D^n. (right? Is there any need of doing this? Just do that in a naive way may be good enough)




4) Prove the high dimensional setting

1) fixed n : small \e, large \e

2) fix \e, study how knee points change as a function of n

3) both n and e change


A key difference in guarantee of Laplacian mechanism and staircase mechanism. If the query output has 2 components, for Laplacian mechanism it only needs to add Laplace noise with parameter D/e to each component, but for staircase mechanism it needs to add staircase distribution with parameter D/e/2 to each component. Which will give us a bad bound in high privacy regime (strictly worse than laplacian mechansim by a factor of 2), and in low privacy regime the cost exponent is -e/4, while the optimal one is -e/3.   




5) Prove the universal result for infinite range and discrete case where delta is 1. Then extend to arbitrary delta case

Seems hard. I don't know how hard it is and I cannot prove it now. Data independent is easy.


Two dimensional search: two way search, for discrete case. at point 0.
